Data Driven Estimation of Stochastic Switched Linear Systems of Unknown Order

We address the problem of learning the parameters of a mean square stable switched linear systems (SLS) with unknown latent space dimension, or \textit{order}, from its noisy input--output data. In particular, we focus on learning a good lower order approximation of the underlying model allowed by finite data. Motivated by subspace-based algorithms in system theory, we construct a Hankel-like matrix from finite noisy data using ordinary least squares. Such a formulation circumvents the non-convexities that arise in system identification, and allows for accurate estimation of the underlying SLS as data size increases. Since the model order is unknown, the key idea of our approach is model order selection based on purely data dependent quantities. We construct Hankel-like matrices from data of dimension obtained from the order selection procedure. By exploiting tools from theory of model reduction for SLS, we obtain suitable approximations via singular value decomposition (SVD) and show that the system parameter estimates are close to a balanced truncated realization of the underlying system with high probability.

==> content/misc.tex <==
\subsection{Regression Estimates}
\label{regression_estimate}
Recall Proposition~\ref{regression_result}, for any sequence $\tl_1^{i}$ of length $i$ the result holds with probability at least $1-\delta$ only if we have $N_{\tl_1^i} \geq \alpha(m + \log{\frac{2}{\delta}})$. The regression estimate for $\tl_1^{i}$ is unreliable when we do not have enough occurrences. In such a case we propose a simple estimate, \textit{i.e.}, we set the regression estimate to $0$. Let us assume we have roll out length of $\hN$, then we need to ensure that for all sequences of length at most $\hN$ the regression estimates hold; in that case by applying a union bound we have that for all sequences simultaneously we have with probability at least $1-\delta$ that $||CA_{\tl_{1}^j}B - \hat{\Theta}_{\tl_{1}^j}||_2 \leq \alpha \beta_{\tl_1^j}\sqrt{\frac{m + \log{\frac{s^{\hN+1}-1}{(s-1)\delta}}}{N_{\tl_1^j}}}$ if $N_{\tl_1^j} \geq \alpha(m + \log{\frac{2(s^{\hN+1}-1)}{(s-1)\delta}})$. The $\frac{s^{\hN+1}-1}{s-1}$ appears because we are taking a union bound over $\frac{s^{\hN+1}-1}{s-1}$ sequences. One observation is that we cannot ensure the high probability bound simultaneously over all sequences up to length $N_S$ because if $\hN = \Theta(N_S)$ then the regression estimate error bound becomes trivial. As a result, we define $N_{up}$ an upper bound for rollout length up to which we can ensure high probability bound. Define a sequence length dependent threshold $\gamma_k = \alpha(m + \log{\frac{2(s^{k+1}-1)}{(s-1)\delta}})$ then 
\begin{align}
    N_{up} = \inf{\{N| N_{\tl_1^{2N}} < \gamma_{2N} \hspace{1.5mm}\forall \tl_1^{2N} \in [s]^{2N}\}}\label{max_rollout}
\end{align}
Intuitively, $2N_{up}$ is the least sequence length such that none of the sequences of that length can be reliably learned by regression, \textit{i.e.}, all sequences with length up to $N_{up}$ occur often enough. Furthermore, since the probability of occurrence decays as the length of the sequence it suggests that no longer sequence can be learned reliably either. We show in Proposition~\ref{n_up} that $N_{up}$ is logarithmic in $N_S$ with high probability. 
With this we can construct an estimate of the system Hankel--like matrix as follows. Let $\hN$ be the rollout length then define
\[
\hat{p}_{\tl_1^i:\tl_1^j} =
\begin{cases}
    \frac{N_{\tl_1^i:\tl_1^j}}{N_S (\hN-i-j+1)} ,& \text{if } i+j > 0\\
    1,              & \text{otherwise}
\end{cases}
\]
$\hat{p}_{\tl_1^i:\tl_1^j}$ is an unbiased estimator for $p_{\tl_1^i:\tl_1^j}$. To see this, recall the experiment set up: we run $N_S$ identical samples of the SLS for length $\hN$. Then for each sample $i \leq N_S$, any sequence $\tl_{1}^k$ can start at position $1, 2, \hdots, \hN-k+1$. Thus for sample $i$ the number of occurrences of $\tl_{1}^k$ is given by $\sum_{l=1}^{N-k+1} \textbf{1}^{(i)}_{\{\tl_1^k \text{starts at position }l\}}$, then $N_{\tl_1^k}$ is given by 
\begin{equation}
N_{\tl_1^k} = \sum_{i=1}^{N_S} \sum_{l=1}^{\hN-k+1} \textbf{1}^{(i)}_{\{\tl_1^k \text{starts at position }l\}}    \label{n_roll}
\end{equation}
and it is clear that $\Ex[N_{\tl_1^k}] = p_{\tl_1^k}N_S (\hN-k+1)$. For the estimates of $CA_{\tl_1^{i}}B$ we have 
\[
\hat{\Theta}_{\tl_1^{i}} =
\begin{cases}
    \text{Regression estimate of Prop.~\ref{regression_result}},& \text{if } N_{\tl_1^{i}} \geq \gamma_{2N_{up}} \\
    0,              & \text{otherwise}
\end{cases}
\]
\begin{align}
[\hHN]_{pL(\tl_{1}^i)+1:pL(\tl_{1}^i)+p , mL(\tl_{1}^j) + 1: mL(\tl_{1}^j)+m} = \sqrt{\hat{p}_{\tl_1^i:\tl_1^j}}\hat{\Theta}_{\tl_1^i:\tl_1^j}   \label{est_hankel_matrix}
\end{align}
The road map for system identification can be summarized as follows. 
\begin{itemize}
\item For a given $N_S$ we do model order selection by choosing two numbers $\hat{N}, r$ which are functions of $N_S$. 
\item Following that we create a finite dimensional estimate $\hHc^{\hat{N}}$ of $\Hci$, and from $\hHc^{\hat{N}}$ we obtain the system parameters of $r$--dimensional approximation of the original SLS using a balanced truncation procedure. 
\item The error between the estimated $r$--dimensional approximation and the true $r$--dimensional approximation can be bounded by subspace perturbation bounds~\cite{sarkar2019finite}.
\end{itemize}
 We now describe details of the balanced truncation below.
 \subsection{Balanced Truncation}
\label{balanced_truncation}
Given the parameters of SLS in Eq.~\eqref{switch_lti} define the following SLS
\begin{align}
    \tx(t+1) &= \sqrt{p_{\theta_t}} A_{\theta_t}\tx(t) + \sqrt{p_{\theta_t}} Bu(t) \nonumber \\
    \ty_t &=   \sqrt{p_{\theta_t}} C\tx(t) \label{sls2}
\end{align}
By our assumption the SLS in Eq.~\eqref{sls2} is strongly stable (See~\cite{petreczky2013balanced}). Now we can use the results in~\cite{birouche2012model} (specifically Eq. ($25$a), ($25$b)). To summarize there exists a linear transformation $S$ such that 
\begin{equation}
S^{\top} X_1 S = S^{-1} X_2 S^{- \top} = \Sigma \label{gramian}    
\end{equation}
where $\Sigma$ is diagonal with entries arranged in descending order, then note that $\Sigma$ satisfies (by definition of $X_1, X_2$)
\begin{equation}
p_i\tilde{A}_i^{\top} \Sigma \tilde{A}_i - \Sigma + p_i\tilde{C}^{\top} \tilde{C} \preceq 0, p_i\tilde{A}_i \Sigma \tilde{A}_i^{\top} - \Sigma +  p_i\tilde{B}\tilde{B}^{\top} \preceq 0  \label{truncation_req}
\end{equation}
where $\tilde{A}_i = S^{\top} A_i  S^{-\top}, \tilde{C} = C S^{-1 \top}, \tilde{B} = S^{\top}B$. Partition $\tilde{A}_i, \tilde{B}, \tilde{C}$ as follows 
\begin{equation}
   \tilde{A}_i = \begin{bmatrix}
    A_i^{(r)} &  \tilde{A}_i^{(12)} \\
     \tilde{A}_i^{(21)} &  \tilde{A}_i^{(22)}
    \end{bmatrix},    \tilde{B}_i = \begin{bmatrix}
    {B}^{(r)} \\
     \tilde{B}^{(2)} 
    \end{bmatrix}, \tilde{C} = [C^{(r)}, \tilde{C}^{(2)}] \label{reduced_model}
\end{equation}
where $A_i^{(r)} \in \Rb^{r \times r}, {B}^{(r)}\in \Rb^{r \times 1}, C^{(r)} \in \Rb^{1 \times r}$ and are the $r$--order balanced truncated version of the true SLS. Then the discussion in Section 4.2 in \cite{birouche2012model} provides error guarantees between the true model and its approximation. Note that in the setting of Section 4.2 in \cite{birouche2012model} $\alpha_i(k) = \sqrt{p}_i \textbf{1}_{\{\theta_k = i\}}$. This observation combined with some linear algebra similar to Section 21.6 of \cite{zhou1996robust} gives us the following proposition.
\begin{proposition}
\label{bt_error_hinf}
Assume $\{\eta_t, w_t\}_{t=1}^{\infty} = 0$. Denote by $M$ the SLS in Eq.~\eqref{switch_lti} and the reduced model corresponding $(\Cr, \{\Ar, p_i\}_{i=1}^s, \Br)$ described in Eq.~\eqref{reduced_model} as $M_r$. $M_r$ is mean square stable and furthermore 
\[
\Delta_{M, M_r} \leq 2\sqrt{s} \sum_{l=r+1}^n \sigma_l
\]
where $\sigma_l$ are the singular values of the Gramian in Eq.~\eqref{gramian}.
\end{proposition}
\begin{proof}
Note that for every $i$ we see $\Sigma$ in Eq.~\eqref{gramian} satisfies Eq.~\eqref{truncation_req}. It can be easily checked that 
\[
p_i\tilde{A}_i^{(r)\top} \Sigma^{(r)} \tilde{A}^{(r)}_i - \Sigma^{(r)} + p_i\tilde{C}^{(r)\top} \tilde{C}^{(r)} \preceq 0, \hspace{1mm} p_i\tilde{A}^{(r)}_i \Sigma^{(r)} \tilde{A}_i^{(r)\top} - \Sigma^{(r)} +  p_i\tilde{B}^{(r)}\tilde{B}^{(r)\top} \preceq 0
\]
where $\Sigma = \begin{bmatrix}
\Sigma^{(r)} & 0 \\
0 & \Sigma^{(2)}
\end{bmatrix}$ and $\Sigma^{(r)}$ is $r \times r$ matrix. Now let $M^{(i)}, M^{(i)}_r$ correspond to $i^{\text{th}}$ subsystem and $r$--order balanced truncated $i^{\text{th}}$ subsystem respectively then $||M^{(i)} - M^{(i)}_r||_{\infty} \leq 2 \sum_{l=r+1}^n \sigma_l$. This means for some $||u||_2 \leq 1$ we have 
\[
||y^{(i)} - y^{(i)}_r||_2 \leq 2 \sum_{l=r+1}^n \sigma_l
\]
where $y^{(i)}, y^{(i)}_r$ is the output response of subsystem $i$ and $r$-order truncated subsystem $i$ respectively to $u$. Then for any $||u||_2 \leq 1$
\begin{align}
\sum_{i=1}^s ||y^{(i)} - y^{(i)}_r||^2_2 \leq 4 s(\sum_{l=r+1}^n \sigma_l)^2 \implies \Delta_{M, M_r}^2 \leq 4s(\sum_{l=r+1}^n \sigma_l)^2
\end{align}
where the final implication follows because each $A_i, B_i, C_i$ is scaled by $\sqrt{p_i}$. 
\end{proof}
\vspace{3mm}
Next, we show how to obtain the reduced order models $(\Cr, \{\Ar\}_{i=1}^s, \Br)$ directly from system Hankel matrix $\Hci$. Recall the SVD from Proposition~\ref{full_rank}, $\Hci = U \Sigma V^{\top}$ where 
\begin{align}
    U\Sigma^{1/2} &= \underbrace{\begin{bmatrix}
    \tC \\
    \sqrt{p_1}\tC \tA_{1} \\ 
    \vdots \\
    \sqrt{p_{\tl_1^{i}}}\tC \tA_{\tl_1^i}\\
    \vdots 
    \end{bmatrix}}_{=\Oc}, \Sigma^{1/2} V^{\top} = \underbrace{[\tB,  \sqrt{p_1}\tA_{1}\tB, \hdots, \sqrt{p_{\tl_1^{i}}}\tA_{\tl_1^i}\tB, \hdots]}_{=\Rc}
\end{align}
with $\Oc^{\top} \Oc = \Rc \Rc^{\top} = \Sigma$. 
\begin{proposition}
\label{r_order_balanced}
Fix $r \leq n$ and $\Hci = U \Sigma V^{\top}$. Then the $r$--order balanced truncated model $(\Cr, \{\Ar\}_{i=1}^s, \Br)$ is given by 
\[
\Cr = [U\Sigma^{1/2}]_{1:p, 1:r}, \Br= [\Sigma^{1/2}V^{\top}]_{1:r, 1:m}
\]
and 
\[
\sqrt{p_i}\Ar = \Sigma^{-1/2}_r U_r^{\top} \Hci_{i} V_r \Sigma^{-1/2}_r
\]
where $U_r, V_r, \Sigma_r$ correspond to top $r$ left singular vectors, right singular vectors and singular values respectively.
\end{proposition}
Proposition~\ref{r_order_balanced} makes it clear that to find $r$--order balanced truncated models we only need top $r$--singular vectors (and singular values). This observation is important because in the presence of finite noisy data estimating singular vectors corresponding to very low singular values typically requires a lot of data. Instead one could focus on simply estimating the significant singular vectors via balanced truncation. Furthermore, the stochastic $L_2$ distance between the original SLS and its $r$--order balanced truncated version is given by Proposition~\ref{bt_error_hinf}. We can now summarize our algorithm below.

%%%%%%%%%%%%%%%
Observe that the Frobenius norm of the difference $\bHhN - \Hci$ can be represented as
 $||\bHhN - \Hci||_F^{2} \leq \sum_{i+j \geq 2\hN -1} p_{\tl_1^i:\tl_1^{j}}||CA_{\tl_1^i:\tl_1^{j}}B||_F^2$. 
Clearly as $\hN$ increases the truncation error decreases. For the case of estimation error we can use Proposition~\ref{regression_result}. Intuitively, it would make sense that $E_{\hN}$ grows with $\hN$ (keeping $N_S$ fixed) as we are trying to estimate a larger matrix. As a result, for large enough $N_S$, there exists $\hN < \infty$ such that $T_{\hN} \leq \alpha E_{\hN}$ for some absolute constant $\alpha \geq 1$. The key idea will be to choose $\hN$ such that $T_\hN \leq \alpha E_\hN$. This idea is formalized in Proposition~\ref{truncation_v_estimation}. Furthermore, for such a choice of $\hN$ we have $||\Hci - \hHhN||_F^2 \leq (1 + \alpha^2) T_\hN^2$ implying that we can estimate the system Hankel matrix well if $T_{\hN}$ is low. 
% Define
% \begin{align}
%     \Ecd_0(N_S) &= \sum_{N_{\tl_1^{k}} < s_0}\frac{||CA_{\tl_1^k}B||_F^2 N_{\tl_1^{k}}}{N_S} \nonumber\\
%     &+2\alpha^2 \hN^2 \sup_{k \leq 2\hN}\sum_{\tl_1^k \in [s]^k}  \frac{||CA_{\tl_1^{k}}B||^2_F(m + \log{\frac{1}{\delta}})}{N_{S}} \nonumber\\
%     \Ecd_1(N_S) &= \alpha^2 \hN^2  \sup_{k \leq 2\hN}\sum_{\tl_{1}^{k} \in [s]^k} \sqrt{\frac{ \hN p_{\tl_1^k}}{ N_S} \log{\Big(\frac{s}{\delta}}\Big)} ||CA_{\tl_1^k}B||^2_F  \label{error_terms}
% \end{align}
% where $s_0 = \alpha (m + \log{\frac{(s^{N+1}-1)}{(s-1)\delta}})$ and $\alpha$ is a known absolute constant.
\begin{proposition}
\label{estimation_error_prop}
Fix $\hN, N_S$ and $\delta$. Then with probability at least $1 -\delta$ we have 
\[
E_\hN = ||\HhN-\hHhN||_F^2 \leq 2\Ecd(N_S) 
\]
with $\Ecd= \alpha^2 \hN^2\frac{\beta^2(m + s_0)}{N_{S}}(\frac{s^{2\hN+1}-1}{s-1})$. Here $\alpha \geq 1$ is a known absolute constant and $s_0 = \log{\frac{(s^{N_{up}+1}-1)}{(s-1)\delta}}$.
\end{proposition}
\begin{proof}
Let $s_0 = \log{\frac{(s^{N_{up}+1}-1)}{(s-1)\delta}}$. By definition we have 
\begin{align}
    [\HhN-\hHhN ]_{L(\tl_1^i), L(\tl_1^j)} &= \sqrt{p_{\tl_1^i:\tl_1^j}}CA_{\tl_1^i:\tl_1^j}B - \sqrt{\hp_{\tl_1^i:\tl_1^j}}\hat{\Theta}_{\tl_1^i:\tl_1^j} \nonumber\\
    &= \underbrace{\Big(\sqrt{p_{\tl_1^i:\tl_1^j}} - \sqrt{\hp_{\tl_1^i:\tl_1^j}} \Big)CA_{\tl_1^i:\tl_1^j}B}_{=\Ec_{1, \tl_{1}^i:\tl_1^{j}}} + \underbrace{\sqrt{\hp_{\tl_1^i:\tl_1^j}}(CA_{\tl_1^i:\tl_1^j}B - \hat{\Theta}_{\tl_1^i:\tl_1^j})}_{=\Ec_{0, \tl_{1}^i:\tl_1^{j}}} \nonumber 
\end{align}
First we analyze $\Ec_{1, \tl_{1}^i:\tl_1^{j}}$. It is clear that 
\begin{align*}
  \sum_{0 \leq i, j \leq \hN-1}||\Ec_{1, \tl_{1}^i:\tl_1^{j}}||_F^2  &\leq \sum_{0 \leq i, j \leq \hN-1}\Big(\sqrt{p_{\tl_1^i:\tl_1^j}} - \sqrt{\hp_{\tl_1^i:\tl_1^j}} \Big)^2 ||CA_{\tl_1^i:\tl_1^j}B||_F^2   \\
  &\leq \sum_{k=0}^{2\hN-2} (k+1)\sum_{\tl_1^k \in [s]^k}\Big(\sqrt{p_{\tl_1^k}} - \sqrt{\hp_{\tl_1^k}} \Big)^2 ||CA_{\tl_1^k}B||_F^2 
\end{align*}
The $k+1$ is the number of times a $k$--length sequence appears in the Hankel--like matrix. Using Proposition~\ref{error_diff} with probability at least $1-\delta$, $\sum_{0 \leq i, j \leq \hN-1}||\Ec_{1, \tl_{1}^i:\tl_1^{j}}||_F^2 \leq \frac{2\alpha \hN^2 \beta^2s_0}{N_S}$. For $\Ec_{0, \tl_1^i:\tl_1^{j}}$ we have
\begin{align*}
    \sum ||\Ec_{0, \tl_1^i:\tl_1^{j}}||_F^2 \leq  \sum_{0 \leq i, j \leq \hN-1} {{\hp_{\tl_1^i:\tl_1^j}}||CA_{\tl_1^i:\tl_1^j}B - \hat{\Theta}_{\tl_1^i:\tl_1^j}||_F^2}
\end{align*}
Recall that whenever $N_{\tl_1^{i}:\tl_{1}^j} <  s_0$, \textit{i.e.}, scarce data, we set $\hat{\Theta}_{\tl_1^i:\tl_1^j} = 0$. Then we get 
\begin{align}
    \sum {{\hp_{\tl_1^i:\tl_1^j}}||CA_{\tl_1^i:\tl_1^j}B - \hat{\Theta}_{\tl_1^i:\tl_1^j}||_F^2} \leq \sum_{N_{\tl_1^{i}:\tl_{1}^j} < s_0} \hp_{\tl_1^i:\tl_1^j}||CA_{\tl_1^i:\tl_1^j}B||_F^2 + \sum_{N_{\tl_1^{i}:\tl_{1}^j} \geq s_0} \hp_{\tl_1^i:\tl_1^j} ||CA_{\tl_1^i:\tl_1^j}B - \hat{\Theta}_{\tl_1^i:\tl_1^j}||_F^2 \label{err0}
\end{align}
We now use Proposition~\ref{regression_result} (applied with union bound to all sequences) with probability at least $1-\delta$
\begin{align}
    \sum_{N_{\tl_1^{i}:\tl_{1}^j} \geq s_0} \frac{N_{\tl_1^i:\tl_1^j}||CA_{\tl_1^i:\tl_1^j}B - \hat{\Theta}_{\tl_1^i:\tl_1^j}||_F^2}{N_S(\hN-i-j+1)} &\leq  \alpha^2 \sum_{N_{\tl_1^{i}:\tl_{1}^j} \geq s_0}  \frac{\beta^2(m + s_0)}{N_{S}(\hN-i-j+1)}   \nonumber \\
    &\leq  \alpha^2 \sum_{k=0}^{2 \hN -2}(k+1)\sum_{\tl_1^k \in [s]^k}  \frac{\beta^2(m + s_0)}{N_{S}(N-k+1)}  \nonumber\\
    &\leq 2\alpha^2 \hN^2 \sup_{k \leq 2\hN}\sum_{\tl_1^k \in [s]^k}  \frac{\beta^2s^{k}(m + s_0)}{N_{S}}\nonumber\\ 
    &\leq  2\alpha^2 \hN^2\frac{\beta^2(m + s_0)}{N_{S}}\Big(\frac{s^{2\hN+1}-1}{s-1}\Big)  \label{err1}
\end{align}
From first part in Proposition~\ref{hoeffding} we get with probability at least $1-\delta$
\begin{align}
\sum_{N_{\tl_1^{i}:\tl_{1}^j} < s_0}{||CA_{\tl_1^i:\tl_1^j}B||_F^2 \hp_{\tl_1^{i}:\tl_{1}^j}} &\leq \frac{2\alpha^2 \hN^2s_0}{N_S} \sup_{k}\sum_{\tl_1^k \in [s]^k} ||CA_{\tl_1^k}B||_F^2 \leq \frac{2\alpha^2 \beta^2 \hN^2s_0}{N_S}
\end{align}
Then combining these observations we get $\sum {{\hp_{\tl_1^i:\tl_1^j}}||CA_{\tl_1^i:\tl_1^j}B - \hat{\Theta}_{\tl_1^i:\tl_1^j}||_F^2} \leq \Ec^{\delta, \hN}$.
\end{proof}
Proposition~\ref{estimation_error_prop} provides an upper bound on $E_\hN^2$ almost entirely in terms of data dependent quantities. From here on we will use $\Ecd(N_S)$ as a proxy for $E_{\hN}^2$. 
%%%%%%%%%%%
% A very loose upper bound on $\Ecd_0, \Ecd_1$ can be obtained by naively upper bounding over all the quantities
% \begin{align*}
%     \Ecd_0(\delta), \Ecd_1(\delta)  &\leq \frac{2 \alpha^2 \hN^2 \beta^2 (\frac{s^{\hN+1}-1}{s-1})(m + \log{\frac{1}{\delta}})}{N_S} 
% \end{align*}
% This suggests $\hN$ needs to depend logarithmically in $N_S$.  However in many cases the dependence is not that dire. Consider the special case of strongly stable SLS, \textit{i.e.}, $\sum_{i=1}^s A_i \otimes A_i$ is Schur stable. In that case $||CA_{\tl_1^{k}}B||_F$ decays exponentially with $k$ and $\sum_{\tl_1^k \in [s]^k}||CA_{\tl_1^{k}}B||^2_F \leq L_0$ where $L_0$ does not depend on $\hN$. Then
% \begin{align*}
%     \Ecd_0(N_S) &= \sum_{N_{\tl_1^{k}} < s_0}\frac{||CA_{\tl_1^k}B||_F^2 N_{\tl_1^{k}}}{N_S} \nonumber\\
%     &+2\alpha^2 \hN \sup_{k \leq 2\hN}\sum_{\tl_1^k \in [s]^k}  \frac{||CA_{\tl_1^{k}}B||^2_F(m + \log{\frac{1}{\delta}})}{N_{S}} \nonumber \\
%     &\leq \frac{\alpha_0^2 \hN^2}{N_S}\Big(m + \log{\frac{1}{\delta}}\Big)
% \end{align*}
% where the last inequality follows from Cauchy Schwartz and $\alpha_0$ is an absolute constant. Then as long as $\hN = o(\sqrt{N_S})$ we can get good finite time estimation error. A similar argument would hold for $\Ecd_1(N_S)$. Instead of using the loose upper bounds a strategy to estimate the error bounds could be to use estimated quantities $\hat{p}_i, \hat{\Theta}_{\tl_1^k}$ to obtain bounds on $p_{\tl_1^k}, \Theta_{\tl_1^k}$. Due to a shortage of space we do not go into the details but refer the reader to~\cite{shawe1998structural} which studies structural risk minimization for data dependent quantities.
%%%%%%%%%%%%
For shorthand $\Ec^{\delta, \hN} = \Ec^{\delta, \hN}(N_S)$. Given this dependence of estimation error on $\hN, N_S$, we find that if we set $\hN$ in a data dependent fashion as follows:
\begin{align}
\hN \overset{\Delta}{=} \hN(N_S)= \inf\Big\{l \bl &||\hHc^{(l)}-\hHc^{(h)}||_F^2 \leq \alpha^2 \beta^2 \Big(\frac{N}{N_S}\Big)(m + \log{\frac{s_{N}}{\delta}}) s_{N} \hspace{1.5mm}\forall N_{up} \geq h \geq l \Big\} \label{data_dep_N}     
\end{align}
where $\alpha_0$ is a known absolute constant and $N_{up}$ is given in Eq.~\eqref{max_rollout}.
\begin{theorem}
\label{thm1}
Fix $\delta > 0$. For large enough $N_S$, pick $\hN$ as in Eq.~\eqref{data_dep_N}. Then with probability at least $1-\delta$ we have 
\[
||\bar{\hHc}^{(\hN)}-\Hci||_F^2 \leq 2 \alpha^2\frac{ \hN^2 s_{2\hN}  \beta^2(m + \log{\frac{s_{N_{up}}}{\delta}})}{N_S} 
\]
where $\bar{\hHc}^{(\hN)}$ is the zero padded version of $\hHc^{(\hN)}$ to make it compatible with $\Hci$ and $\alpha \geq 1$ is an absolute constant. Here $s_{k} =\frac{s^{k+1}-1}{s-1}$.
\end{theorem}
\begin{proof}
We sketch the details of the proof here. We assume all matrices are size compatible by padding with zeros. The large enough $N_S$ is required only to ensure that there exists $\hN < \infty$ such that $T_{\hN} \leq \Ec^{\delta, \hN}$. Define $\hN^{*} = \inf{\{N| T_N \leq \Ec^{\delta, N}\}}$. In general $\hN^{*}$ is unknown as it is complex function of unknown system parameters (because of $T_N$). By Proposition~\ref{truncation_v_estimation} such $\hN^{*}$ exists. However, by leveraging results from~\cite{sarkar2019finite} specifically Proposition 12.1 and 12.2 we can show that 
\[
\hN(N_S) \leq \hN^{*} \leq \log{(\alpha_0)} \hN(N_S)
\]
with probability at least $1 - \delta$. We show $\hN^{*} \geq \hN(N_S)$ in Proposition~\ref{lb_hn}. The other inequality follows the same steps as Prop 12.2 in~\cite{sarkar2019finite}. Based on this observation we note for any $l  \geq \hN$
\begin{align*}
       \sqrt{\alpha_0 {\Ec}^{\delta, \hNs}} \geq ||\hHhN - \hHc^{(\hNs)}||_F \geq    ||\hHhN - \Hci||_F - ||\Hci - \hHc^{(\hNs)}||_F
\end{align*}
This gives
\begin{align*}
  & ||\hHhN - \Hci||_F \leq \sqrt{\alpha_0 {\Ec}^{\delta, \hNs} } + ||\Hci - \hHc^{(\hNs)}||_F
\end{align*}
Since $E_{\hNs} \geq T_{\hNs}$ we have that $||\hHc^{(\hNs)} - \hHc^{(\hNs)}||_F \leq 2 {\Ec}^{\delta, \hNs}$. Then it implies that 
\begin{equation}
||\hHhN - \Hci||^2_F \leq (\alpha_0 + 2) {\Ec}^{\delta, \hNs}  \label{data_error}   
\end{equation}
Our claim follows by noting that ${\Ec}^{\delta, \hNs}  \leq {\Ec}^{\delta, \log{(\alpha_0)} \hN}$. \qed
\end{proof}
The key insight of Theorem~\ref{thm1} is that for the choice of $\hN(N_S)$ in Eq.~\eqref{data_dep_N} we can get a good upper bound on the error between the true system Hankel matrix, $\Hci$, and its estimate $\hHhN$. Furthermore this bound does not depend on the system order, $n$, but only data dependent quantities and some energy metrics which can be measured easily. The result in Proposition~\ref{truncation_v_estimation} (and Eq.~\eqref{est_error}) shows that
\begin{equation}
  ||\bar{\hHc}^{(\hN)} - \Hci||^2_F  = O(N^{-\delta_s}) \label{error_rate}
\end{equation}
where $\delta_s = \Big(\log{\frac{1}{p_{\max}}}\Big)\Big({\log{\frac{s}{p_{\max}}}}\Big)^{-1}$. Eq.~\eqref{error_rate} shows that decay in error between the true system Hankel--like matrix and its estimator is roughly $\frac{1}{\sqrt{N_S^{-\delta_s}}}$ (ignoring the log factors) and the error between $\bar{\hHc}^{(\hN)}, \Hci$ goes to zero asymptotically as $N_S \rightarrow \infty$. 


==> content/n_select.tex <==
\section{Choosing the rollout length}
\label{sec:n_select}
As we discussed in Section~\ref{sec:N_NS}, the rollout length $N$ is needed to estimate the ``mixing'' properties of the SLS. 
